The full four-loop cusp anomalous dimension in $\mathcal{N}=4$ super Yang-Mills and QCD

We present the complete formula for the cusp anomalous dimension at four loops in QCD and in maximally supersymmetric Yang-Mills. In the latter theory it is given by \begin{equation} {\Gamma}^{\rm}_{\rm cusp}\Big|_{\alpha_s^4} = -\left( \frac{\alpha_s N}{\pi}\right)^4 \left[ \frac{73 \pi^6}{20160} + \frac{ \zeta_{3}^2}{8} + \frac{1}{N^2} \left( \frac{31\pi^6}{5040} + \frac{9 \zeta_3^2}{4} \right) \right] \,.\nonumber \end{equation} Our approach is based on computing the correlation function of a rectangular light-like Wilson loop with a Lagrangian insertion, normalized by the expectation value of the Wilson loop. In maximally supersymmetric Yang-Mills theory, this ratio is a finite function of a cross-ratio and the coupling constant. We compute it to three loops, including the full colour dependence. Integrating over the position of the Lagrangian insertion gives the four-loop Wilson loop. We extract its leading divergence, which determines the four-loop cusp anomalous dimension. Finally, we employ a supersymmetric decomposition to derive the last missing ingredient in the corresponding QCD result.

==> Plots/Dia_RAAA.tex <==
\begin{tikzpicture}[scale=0.8, baseline=(current bounding box.center)]
% >>>>>>>>>>>>> CR CA^3 <<<<<<<<<<<

      \node at (0,0) {~};
      \node at (0,-2.1) {~};

      \coordinate (WL) at (-2,-2)   {};
      \coordinate (cusp) at (0,0)   {};
      \coordinate (WR) at (2,-2) {};
      
      \coordinate (B1) at (-0.5,-1.9) {};
      \coordinate (B2) at (+0.5,-1.9) {};
      \coordinate (B3) at (-0.3,-1.2) {};

      
      \coordinate (W1) at (-1.6,-1.6) {};
      \coordinate (W2) at (-0.5,-0.5) {};
      \coordinate (W3) at (0.5, -0.5) {};
      \coordinate (W4) at (1.1, -1.1) {};
      \coordinate (W5) at (1.6, -1.6) {};
      
      \draw[Wilson_1] (WL)  -- (cusp) -- (WR);
      
      \draw[Gluon_1] (B1) -- (W1) ;
      \draw[Gluon_1] (B2) -- (B1) ;
      \draw[Gluon_1] (W5) -- (B2) ;
      \draw[Gluon_1] (W2) -- (B3) ;
      \draw[Gluon_1] (B1) -- (B3) ;
      \draw[Gluon_1] (B2) .. controls (0.7,-1.4) .. (W4) ;
      \draw[Gluon_1] (W3) .. controls (0.3,-0.9) .. (B3) ;
      
      
\end{tikzpicture}


==> Plots/Dia_dRdA.tex <==
\begin{tikzpicture}[scale=0.8, baseline=(current bounding box.center)]
% >>>>>>>>>>>>> dR dA <<<<<<<<<<<
      
      \node at (0,0) {~};
      \node at (0,-2.1) {~};
      
      \coordinate (WL) at (-2,-2)   {};
      \coordinate (cusp) at (0,0)   {};
      \coordinate (WR) at (2,-2) {};
      
      \coordinate (W1) at (-1.6,-1.6) {};
      \coordinate (W2) at (-1.2,-1.2) {};
      \coordinate (W3) at (-0.7, -0.7) {};
      \coordinate (W4) at (-0.3, -0.3) {};
      \coordinate (W5) at (0.3, -0.3) {};
      \coordinate (W6) at (0.7, -0.7) {};
      \coordinate (W7) at (1.2,-1.2) {};
      \coordinate (W8) at (1.6,-1.6) {};
      
      \draw[Wilson_1] (WL)  -- (cusp) -- (WR);
      
      
      \draw[Gluon_1] (W6) .. controls (-0.3,-1.2) .. (W2) ;
      \draw[white,fill=white] (0,-1.05) circle (8pt);
      \draw[Gluon_1] (W7) .. controls (0.3,-1.2) .. (W3) ;
      \draw[white,fill=white] (0.01,-1.05) circle (6.1pt);
      \draw[Gluon_1] (W5) .. controls (-0.1,-1.4) .. (W1) ;
      \draw[white,fill=white] (-0.025,-1.045) circle (4pt);
      \draw[Gluon_1] (W8) .. controls (0.1,-1.4) .. (W4) ;
      
\end{tikzpicture}


==> Plots/Dia_fdRdF.tex <==
\begin{tikzpicture}[scale=0.8, baseline=(current bounding box.center)]
% >>>>>>>>>>>>> nf dRdF <<<<<<<<<<<

      \node at (0,0) {~};
      \node at (0,-2.1) {~};

      \coordinate (WL) at (-2,-2)   {};
      \coordinate (cusp) at (0,0)   {};
      \coordinate (WR) at (2,-2) {};
      
      \coordinate (B1) at (-0.4,-1.1) {};
      \coordinate (B2) at (0.4,-1.1) {};
      \coordinate (B3) at (0.4,-1.9) {};
      \coordinate (B4) at (-0.4,-1.9) {};
      
      \coordinate (W1) at (-0.8,-0.8) {};
      \coordinate (W4) at (-1.257,-1.257) {};
      \coordinate (W2) at (0.8,-0.8) {};
      \coordinate (W3) at (1.257,-1.257) {};
      
      \draw[Wilson_1] (WL)  -- (cusp) -- (WR);
      \draw (B1) -- (B2) -- (B3) -- (B4) -- (B1);
      \draw[Gluon_1] (B1) -- (W1) ;
      \draw[Gluon_1] (B4) -- (W4) ;
      \draw[Gluon_1] (W3) -- (B3) ;
      \draw[Gluon_1] (W2) -- (B2) ;
\end{tikzpicture}

